Liftago On-Demand Transport Dataset and Market Formation Algorithm Based on Machine Learning

This document serves as a technical report for the analysis of on-demand transport dataset. Moreover we show how the dataset can be used to develop a market formation algorithm based on machine learning. Data used in this work comes from Liftago, a Prague based company which connects taxi drivers and customers through a smartphone app. The dataset is analysed from the machine-learning perspective: we give an overview of features available as well as results of feature ranking. Later we propose the SImple Data-driven MArket Formation (SIDMAF) algorithm which aims to improve a relevance while connecting customers with relevant drivers. We compare the heuristics currently used by Liftago with SIDMAF using two key performance indicators.

==> secIntro.tex <==
\section{Introduction}

Catching a taxi has changed over the last few years. In New York City at the turn of the millennium, hailing a cab from the side of the road was the norm. Or in Sydney, it was common to call a taxi dispatcher for a journey to the airport. Now in 2016 it is increasingly common to instead open an app on a smartphone to book transport via Uber\footnote{\url{https://www.uber.com/}}, Lyft\footnote{\url{https://www.lyft.com/}}, or one of several other on-demand transport services.

What has changed? After the now widespread adoption of internet-enabled smartphones and secure online payments, it is possible for both potential passengers and drivers to easily communicate with a provider or directly with each other. This offers the potential for passengers to be transported, irrespective of their location and the locations of available drivers. The problem that remains is to determine which driver should transport which passenger, known as the allocation.

The high level of connectivity that we now take for granted also offers the means to help with the allocation problem. In particular, the use of smartphone apps has made it possible for providers to collect huge amounts of data, such as the time and location of passenger pick-ups or drop-offs, as well as the prices passengers are prepared to pay and the fares drivers are willing to accept. The combination of this data is leading to new insights into the spatial-temporal profile of on-demand transport systems and ultimately opens the way for increasingly efficient allocation and pricing.

However, coping with the size of the data and developing methods to combine different data sets raise new challenges. It is here that techniques from machine learning are playing an important role, ranging from helping empty vehicles find locations with high densities of passengers \cite{Moreira-Matias2013} to solving the allocation and pricing problems.

In fact, data-driven allocation and pricing is now an active area of research and plays a key role in real-world on-demand transport services. By accounting for the real-time behavior of passengers and drivers, it is possible to improve the reliability of on-demand transport services in terms of waiting times, driver profits, and also provider revenue.

In this paper, we survey a range of data-driven on-demand transport allocation schemes that have been recently proposed and provide a classification to identify the strengths of each scheme as well as open problems. In particular, our classification is based on the fact that the allocation schemes are different variants of two-sided markets. As such, each allocation scheme can be viewed as an implementation of a market mechanism from economics in the context of on-demand transport.

While many aspects of how to allocate and price passengers are now understood, a key difficulty that remains in applying market mechanisms to on-demand transport is how to form the market; that is, which drivers and passengers should be allowed to be matched. Clearly, the distances from each passenger to each driver impose important constraints, however further features can be considered to improve the efficiency of the matching.

To explore the effect of different features in the market formation step of the allocation, we apply feature extraction techniques from machine learning to a real-world data set. Our data set is obtained from the on-demand transport provider Liftago\footnote{\url{https://www.liftago.com/}}, which operates in Prague, Czech Republic. Using this data set, we show that while passenger-driver distance is a key feature, a number of other features play a key role. These features include individual driver behavior and spatial-temporal information such as time of day and the location of pick-up. Ultimately, data-driven market formation in concert with the data-driven allocation schemes form a toolbox to assist on-demand transport providers to structure their services.

